$\textit{Ab initio}$-guided X-ray photoelectron spectroscopy quantification of Ti vacancies in Ti$_{1-\delta}$O$_x$N$_{1-x}$ thin films

$\textit{Ab initio}$ calculations were employed to investigate the effect of oxygen concentration dependent Ti vacancies formation on the core electron binding energy shifts in cubic titanium oxynitride (Ti$_{1-\delta}$O$_x$N$_{1-x}$). It was shown, that the presence of a Ti vacancy reduces the 1s core electron binding energy of the first N neighbors by $\sim$0.6 eV and that this effect is additive with respect to the number of vacancies. Hence it is predicted that the Ti vacancy concentration can be revealed from the intensity of the shifted components in the N 1s core spectra region. This notion was critically appraised by fitting the N 1s region obtained via X-ray photoelectron spectroscopy (XPS) measurements of Ti$_{1-\delta}$O$_x$N$_{1-x}$ thin films deposited by high power pulsed magnetron sputtering. A model to quantify the Ti vacancy concentration based on the intensity ratio between the N 1s signal components, corresponding to N atoms with locally different Ti vacancy concentration, was developed. Herein a random vacancy distribution was assumed and the influence of surface oxidation from atmospheric exposure after deposition was considered. The so estimated vacancy concentrations are consistent with a model calculating the vacancy concentration based on the O concentrations determined by elastic recoil detection analysis and text book oxidation states and hence electroneutrality. Thus, we have unequivocally established that the formation and population of Ti vacancies in cubic Ti$_{1-\delta}$O$_x$N$_{1-x}$ thin films can be quantified by XPS measurements from N 1s core electron binding energy shifts.

==> Makefile <==
.PHONY: all clean figures

ARTICLE = TiON-XPS-DFT

all: $(ARTICLE).pdf Z-TiON-XPS-DFT-SM.pdf

$(ARTICLE).pdf: $(ARTICLE).tex figures bib-db.bib XPS-table.tex
	pdflatex $(ARTICLE).tex; \
	pdflatex $(ARTICLE).tex; \
	bibtex $(ARTICLE); \
	pdflatex $(ARTICLE).tex; \

%.rtf: %.tex figures rtfhead.tex XPS-table.tex
	cat rtfhead.tex >tmp.tex
	tail -n +2 $*.tex >> tmp.tex
	sed -i 's/elsarticle-num/unsrt/g' tmp.tex
	sed -i 's/\[MCh\]/\[1\]/g' tmp.tex
	sed -i 's/\[Leoben\]/\[2\]/g' tmp.tex
	sed -i 's/\[Uppsala\]/\[3\]/g' tmp.tex
	sed -i 's/^\\address/\\affil/g' tmp.tex
	sed -i '/^\\cortext/d' tmp.tex
	pdflatex tmp.tex
	pdflatex tmp.tex
	bibtex tmp
	pdflatex tmp.tex
	latex2rtf -Z1 -M12 tmp.tex
	mv tmp.rtf $@
	#rm tmp.*

Z-TiON-XPS-DFT-SM.pdf: Z-TiON-XPS-DFT-SM.tex figures bib-db.bib ERDA-table.tex
	@if [ $$(ls --sort=time figures/* | head -n1) -nt Z-TiON-XPS-DFT-SM.pdf ] || [ "$?" != "figures" ]; then \
		rm -f Z-TiON-XPS-DFT-SM.tmp; \
		while ! cmp --quiet Z-TiON-XPS-DFT-SM.aux Z-TiON-XPS-DFT-SM.tmp; do \
			cp Z-TiON-XPS-DFT-SM.aux Z-TiON-XPS-DFT-SM.tmp; \
			pdflatex Z-TiON-XPS-DFT-SM.tex; \
			if grep -q '^\\bibliography' "Z-TiON-XPS-DFT-SM.tex"; then \
				bibtex Z-TiON-XPS-DFT-SM; \
			fi; \
		done; \
		rm -f Z-TiON-XPS-DFT-SM.tmp; \
	fi

ERDA-table.tex: figures/data/ERDA.txt
	rm -f $@
	sort -n -k 4 $< | awk 'function translate(b){if (b == 3395) return 0; if (b == 3396) return 0.45; if (b == 3397) return 0.9; if (b == 3398) return 1.35;}{if(NR > 1){printf "%.2f & %.1f & %.1f $$\\pm$$ %.1f & %.1f $$\\pm$$ %.1f & %.1f $$\\pm$$ %.1f & %.3f \\\\\n", translate($$1), $$2*4.3-0.1, $$3, $$6, $$4, $$7, $$5, $$8, $$4/($$4+$$5)}}'  >> $@
	sed -i '$$s/..$$//' $@

XPS-table.tex: figures/data/XPS/XPS-fit-results.txt
	rm -f $@
	awk '{if (NR == 1) next; sum = ($$8 + $$14 + $$20 + $$26 + $$32)/100; printf "%.1f & %.1f & %.1f & %.1f & %.1f & %.1f & %.2f & %.2f & %.2f & %.2f & %.2f & %.2f & %.2f \\\\\n", $$3, $$8/sum, $$14/sum, $$20/sum, $$26/sum, $$32/sum, $$10, $$16, $$22, $$28, $$34, $$10-$$16, $$16-$$22}' $< > $@
	sed -i '$$s/..$$//' $@

figures:
	$(MAKE) -C $@

clean:
	rm -f *.aux *.log *.out *~ *.pdf *.bbl *.blg ERDA-table.tex
	$(MAKE) -C figures $@


==> figures/Makefile <==
.PHONY: all clean

FIGURES = XPS-spectra-total.pdf TiON-latpar.pdf TiON-Ef.pdf expshifts.pdf N1s-peak-intensities.pdf TiON-vac.pdf N1s-TiON.pdf N1s-peak-intensities.pdf DFT-spectra-selected.pdf XRD-over.pdf fit-N1s-TiON-all.pdf

SIGMA = 0.3

all: $(FIGURES)

%.pdf: %.gpi
	gnuplot $< > $@

%.pdf: %.svg
	inkscape --without-gui --export-pdf=$@ --file=$<
	
SQSSOURCEDIR = sl119982@login18-1.hpc.itc.rwth-aachen.de:/work/sl119982/TiON-balanced/Wien2k
SQSDIR = data/SQS
	
SQSXS = 0.09375 0.1875 0.28125 0.375 0.46875
SQSVARS = 0 12 25
SQSALL = $(foreach X, $(SQSXS), $(foreach VAR,$(SQSVARS), $(X)_$(VAR)))
SQSNSTATS = $(patsubst %, $(SQSDIR)/y_%/N-stats.txt, $(SQSALL))
SQSOSTATS = $(patsubst %, $(SQSDIR)/y_%/O-stats.txt, $(SQSALL))
SQSTISTATS = $(patsubst %, $(SQSDIR)/y_%/Ti-stats.txt, $(SQSALL))
SQSALLSTATS = $(SQSNSTATS) $(SQSOSTATS) $(SQSTISTATS)
SQSIMPSPECTRA = $(subst stats,XPS-spectra-imp, $(SQSALLSTATS))
SQSSPECTRA = $(subst stats,XPS-spectra, $(SQSALLSTATS))
SQSALLSPECTRA = $(SQSIMPSPECTRA) $(SQSSPECTRA)

SQSNAIMSTATS = $(patsubst %, $(SQSDIR)/y_%/N-bader-stats.txt, $(SQSALL))
SQSOAIMSTATS = $(patsubst %, $(SQSDIR)/y_%/O-bader-stats.txt, $(SQSALL))
SQSTIAIMSTATS = $(patsubst %, $(SQSDIR)/y_%/Ti-bader-stats.txt, $(SQSALL))
SQSAIMSTATS = $(SQSNAIMSTATS) $(SQSOAIMSTATS) $(SQSTIAIMSTATS)

SQSPARSEDSTATS = $(SQSDIR)/N-total.txt $(SQSDIR)/O-total.txt $(SQSDIR)/Ti-total.txt $(SQSDIR)/N-part.txt
SQSPARSEDAIMSTATS = $(SQSDIR)/N-bader-total.txt $(SQSDIR)/O-bader-total.txt $(SQSDIR)/Ti-bader-total.txt $(SQSDIR)/N-bader-part.txt

$(SQSDIR)/y_%/Ti-stats.txt $(SQSDIR)/y_%/O-stats.txt $(SQSDIR)/y_%/N-stats.txt \
$(SQSDIR)/y_%/N-XPS-spectra-imp.txt $(SQSDIR)/y_%/Ti-XPS-spectra-imp.txt $(SQSDIR)/y_%/O-XPS-spectra-imp.txt: $(SQSDIR)/y_%/*.struct $(SQSDIR)/y_%/XPS-shifts-dscf-cond.txt  $(SQSDIR)/cutoffs.txt
	cd $(SQSDIR)/y_$*; XPS-parse -s -b $(SIGMA) -cf ../cutoffs.txt -geom y_$*.struct XPS-shifts-dscf-cond.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/3/N^{3V_{Ti}}/g' N-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/4/N^{2V_{Ti}}/g' N-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/5/N^{1V_{Ti}}/g' N-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/6/N^{0V_{Ti}}/g' N-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/3/O^{3V_{Ti}}/g' O-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/4/O^{2V_{Ti}}/g' O-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/5/O^{1V_{Ti}}/g' O-XPS-spectra-imp.txt
	cd $(SQSDIR)/y_$*; sed -iE '1 s/6/O^{0V_{Ti}}/g' O-XPS-spectra-imp.txt
 
$(SQSDIR)/y_%/Ti-bader-stats.txt $(SQSDIR)/y_%/O-bader-stats.txt $(SQSDIR)/y_%/N-bader-stats.txt: $(SQSDIR)/y_%/*.struct $(SQSDIR)/y_%/aim.txt $(SQSDIR)/cutoffs.txt
	cd $(SQSDIR)/y_$*; aim-parse -cf ../cutoffs.txt -geom y_$*.struct aim.txt

$(SQSPARSEDAIMSTATS): $(SQSAIMSTATS)
	./parse-aim.sh

$(SQSPARSEDSTATS): $(SQSALLSTATS) data/SQS/parse.sh
	cd data/SQS; ./parse.sh
	
XPS-spectra-total.pdf: $(SQSIMPSPECTRA)

data/XRD/latpar.txt: data/XRD/geta.sh data/XRD/fit-XRD-stress.gpi data/ERDA.txt
	cd data/XRD; bash ./geta.sh

data/XRD/vacancies-XRD.txt: data/XRD/TiON-fitvac-latpar.gpi data/XRD/latpar.txt data/XRD/runvaclatpar.sh data/XRD/XRD-fit.txt
	cd data/XRD; bash ./runvaclatpar.sh
	
data/SQS/DFTlatpar.txt: $(patsubst %, $(SQSDIR)/y_%/*.struct, $(SQSALL))
	rm -f $@
	for f in $^;\
	do\
		X=$$(grep -o "[0-9]*\.[0-9]*" <<< $$f | head -n1);\
		printf "$$X " >> $@;\
		awk '{if (NR == 4) print ($$1 + $$2 + $$3) * 0.529177249 / 2.0 / 3.0}' $$f >> $@;\
	done

#data/ERDA-N2-corrected.txt: data/fix-ERDA.sh data/ERDA.txt data/XPS/XPS-fit-results-tmp.txt
#	bash data/fix-ERDA.sh
	
TiON-latpar.pdf data/XRD/XRD-fit.txt: TiON-latpar.gpi data/XRD/latpar.txt data/SQS/a-SQS.txt data/SQS/a-SQS+1.txt data/SQS/a-SQS+2.txt data/SQS/a-SQS+4.txt
	gnuplot $< > $@

TiON-Ef.pdf: data/SQS/EfSQS.txt data/SQS/EfSQS+1.txt data/SQS/EfSQS+2.txt data/SQS/EfSQS+4.txt

XRD-over.pdf: data/ERDA.txt

XRDCLEAN = data/XRD/latpar.txt data/XRD/fits data/XRD/vacancies-XRD.txt data/XRD/vacfits data/XRD/XRD-fit.txt
XPSCLEAN = data/XPS/XPS-fit-results-tmp.txt data/XPS/XPS-fit-results.txt data/XPS/XPS-fit-results-for-fit.txt data/XPS/c.txt data/XPS/N1s-peak-intensities-fit.pdf data/XPS/vacancies-XPS.txt data/XPS/vacfits
#ERDACLEAN = data/ERDA-N2-corrected.txt

expshifts.pdf: data/XPS/XPS-fit-results.txt $(SQSDIR)/N-part.txt $(SQSDIR)/N-TiN-part.txt

N1s-peak-intensities.pdf: data/XPS/XPS-fit-results.txt

TiON-vac.pdf: data/XRD/vacancies-XRD.txt data/XPS/vacancies-XPS.txt

#data/XPS/XPS-fit-results-tmp.txt: data/XPS/fit.py data/ERDA.txt
#	cd data/XPS; ./fit.py -E ../ERDA.txt; mv XPS-fit-results.txt XPS-fit-results-tmp.txt

data/XPS/XPS-fit-results.txt: data/XPS/fit.py data/ERDA.txt
	cd data/XPS; mkdir fits; ./fit.py -o -E ../ERDA.txt

#this is data file for the fit of the three components to determine the constant offsets
data/XPS/XPS-fit-results-for-fit.txt: data/XPS/extract.sh data/XPS/XPS-fit-results.txt
	bash $< 

data/XPS/N1s-peak-intensities-fit.pdf data/XPS/c.txt: data/XPS/XPS-fit-results-for-fit.txt

data/XPS/vacancies-XPS.txt: data/XPS/runvacXPS.sh data/XPS/N1s-peak-intensities-fit.pdf data/XPS/c.txt
	cd data/XPS; bash runvacXPS.sh

update_data:
	for c in $(SQSALL); do \
		mkdir -p "data/SQS/y_$$c"; \
		scp $(SQSSOURCEDIR)/y_$$c/XPS-shifts-dscf-cond.txt data/SQS/y_$$c/; \
		scp $(SQSSOURCEDIR)/y_$$c/aim.txt data/SQS/y_$$c/; \
		scp $(SQSSOURCEDIR)/y_$$c/y_$$c.struct data/SQS/y_$$c/; \
	done;

clean:
	rm -rf *~ $(FIGURES) $(SQSALLSTATS) $(SQSPARSEDSTATS) $(SQSALLSPECTRA) $(XRDCLEAN) $(XPSCLEAN) $(ERDACLEAN)


==> figures/data/XPS/spectra/TiON <==
z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0001.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0002.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0003.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0004.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0005.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0006.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0007.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0008.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0009.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0010.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0011.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0012.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0013.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0014.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0015.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0016.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0017.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0018.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0019.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0020.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0021.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0022.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0023.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0024.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0025.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0026.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0027.txt
1: N1s


z:\home\ondracka\documents\work\clanky\tion-xps-dft\figures\data\xps\spectra\tion0028.txt
1: N1s



